Adversarial Speaker Disentanglement Using Unannotated External Data for Self-supervised Representation Based Voice Conversion

Nowadays, recognition-synthesis-based methods have been quite popular with voice conversion (VC). By introducing linguistics features with good disentangling characters extracted from an automatic speech recognition (ASR) model, the VC performance achieved considerable breakthroughs. Recently, self-supervised learning (SSL) methods trained with a large-scale unannotated speech corpus have been applied to downstream tasks focusing on the content information, which is suitable for VC tasks. However, a huge amount of speaker information in SSL representations degrades timbre similarity and the quality of converted speech significantly. To address this problem, we proposed a high-similarity any-to-one voice conversion method with the input of SSL representations. We incorporated adversarial training mechanisms in the synthesis module using external unannotated corpora. Two auxiliary discriminators were trained to distinguish whether a sequence of mel-spectrograms has been converted by the acoustic model and whether a sequence of content embeddings contains speaker information from external corpora. Experimental results show that our proposed method achieves comparable similarity and higher naturalness than the supervised method, which needs a huge amount of annotated corpora for training and is applicable to improve similarity for VC methods with other SSL representations as input.

==> text/related_works.tex <==
\subsection{Language}

All manuscripts must be in English.

\subsection{Paper length}

Papers should be no longer than 6 pages, including all text, figures, and references.

\subsection{Supplemental material}

Authors may optionally upload supplemental material. Typically, this material might include:
\begin{itemize}
  \item a short presentation summarizing the paper,
  \item videos of results that cannot be included in the main paper,
  \item screen recording of the running program
  \item anonymized related submissions to other conferences and journals, and
  \item appendices or technical reports containing extended proofs and mathematical derivations that are not essential for understanding of the paper.
\end{itemize}

Note that the contents of the supplemental material should be referred to appropriately in the paper and that reviewers are not obliged to look at it.

All supplemental material must be zipped into a single file. There is a 20MB limit on the size of this file.




Many authors misunderstand the concept of anonymizing for blind review. Blind review does not mean that one must remove citations to one's own work-in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work. That is all. (But see below for technical reports)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith, it says that you are building on her work. If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]''and at the end of the paper, include reference 7 as you would any other cited work.
If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work. In such cases, include the anonymized parallel submission~\cite{Authors12} as additional material and cite it as

\begin{quote}
1. Authors. ``The frobnicatable foo filter'', ACM MM 2016 Submission ID 324, Supplied as additional material {\tt acmmm13.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report. For conference
submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a technical report for further details. Thus, you may say in
the body of the paper ``further details may be found in~\cite{Authors12b}''.  Then submit the technical report as additional material. Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which is widely known to be restricted to a single institution.  For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the ICME audience would like to hear about your solution.  The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus.

You can handle this paper like any other.  Don't write ``We show how to improve our previous work [Anonymous, 1968].  This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''. That would be silly, and would immediately identify the authors. Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}

As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors. A reviewer might think it likely that the new paper was written by Zeus, but cannot make any decision based on that guess. He or she would have to be sure that no other authors could have been contracted to solve problem B.

FAQ: Are acknowledgements OK?  No. Please omit them in the review copy and leave them for the final, camera ready copy.
